Vision+X: A Survey on Multimodal Learning in the Light of Data

We are perceiving and communicating with the world in a multisensory manner, where different information sources are sophisticatedly processed and interpreted by separate parts of the human brain to constitute a complex, yet harmonious and unified sensing system. To endow the machines with true intelligence, multimodal machine learning that incorporates data from various sources has become an increasingly popular research area with emerging technical advances in recent years. In this paper, we present a survey on multimodal machine learning from a novel perspective considering not only the purely technical aspects but also the intrinsic nature of different data modalities. We analyze the commonness and uniqueness of each data format mainly ranging from vision, audio, text, and motions, and then present the methodological advancements categorized by the combination of data modalities, such as Vision+Text, with slightly inclined emphasis on the visual data. We investigate the existing literature on multimodal learning from both the representation learning and downstream application levels, and provide an additional comparison in the light of their technical connections with the data nature, e.g., the semantic consistency between image objects and textual descriptions, and the rhythm correspondence between video dance moves and musical beats. We hope that the exploitation of the alignment as well as the existing gap between the intrinsic nature of data modality and the technical designs, will benefit future research studies to better address a specific challenge related to the concrete multimodal task, prompting a unified multimodal machine learning framework closer to a real human intelligence system.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/dataset.tex <==
\section{Multimodal Datasets}
\label{sec:dataset}

Datasets play an essential role in deep learning research but in the context of multimodal learning, the datasets usually require data and annotations that cover several modalities.
In this section, we summarize different multimodal datasets, categorized by their real-world or synthetic natures, and introduce their basic information including the data scale, annotations, and applicable tasks.
Table~\ref{tab:data} lists the overall information for the presented multimodal datasets.


% \begin{table*}[ht]
%     \centering
%     \scalebox{1.0}{
%     \begin{tabular}{ccccccc}
%     \hline
%         Dataset & Nature & Vision & Audio & Text & Others & Typical Applications  \\ \hline
%         MSCOCO~\cite{lin2014microsoft} & R & image & - & caption & body keypoints &  image captioning 
%         /text-to-image synthesis\\
%         CC~\cite{sharma2018conceptual,changpinyo2021conceptual} & R & image & - & caption & -  & image-text \\
%         CUB200~\cite{WahCUB_200_2011} & R & image & - & caption & -  & text-to-image synthesis \\
%         VisDial~\cite{davis2018visual} & R & image & - & dialog & - & visual dialog \\
%         GuessWhat~\cite{de2017guesswhat}& R & image & - & dialog & - & visual dialog\\
%         NExT-QA~\cite{xiao2021next} & R & video & - & dialog & - & VQA \\
%         MSVD~\cite{chen2011collecting} & R & video & - & caption & - & video captioning \\
%         MSR-VTT~\cite{xu2016msr} & R & video & - & caption & - & video captioning \\ 
%         AVSD~\cite{hori2019end,alamri2019audio} & R & video & ambient & dialog & - & video captioning and visual dialog \\
%         AVE~\cite{tian2018audio} & R & video & ambient & - & & audio-visual event localization\\
%         AIST~\cite{aist-dance-db} & R & video &  music & - & - & dance-music\\
%         AIST++~\cite{aistplus} & R & video & music & - & 2D/3D/SMPL  & dance-music \\
%         TikTok Dance-Music~\cite{yezhu2022quantizedgan}& R & video & music & - & 2D & dance-music \\ 
%         MUSIC~\cite{zhao2018sound,zhao2019sound} & R & video & music & - & - &  video-music\\
%         FACC~\cite{harwath2015deep} & R & image & speech & caption & - & sanity check for multimodal learning\\
%         LLP~\cite{tian2020avvp} & R & video & ambient & - & - & audio-visual video parsing \\
%         CLVER~\cite{johnson2017clevr} & S & image & - & dialog & scene graph &  visual question answering\\
%         MUGEN~\cite{hayes2022mugen} & S & video & music & caption & -  & video-music-text \\
%         \hline
%     \end{tabular}}
%     \caption{\textbf{Overview of various existing multi-modal datasets.} \emph{R} and \emph{S} indicates the real-world and synthetic natures, respectively.  We only list the typical applications related to multi- and cross-modality problems in this table. Some large-scale benchmark dataset such as MSCOCO are also widely used for other tasks such as object segmentation and detection.}
%     \label{tab:data}
% \end{table*}


\vspace{-0.1in}
\subsection{Real-World Dataset}
\label{subsec:real_data}

The real-world data are essential for multimodal networks to be applied in practical scenarios. 


\noindent \textbf{MSCOCO} dataset~\cite{lin2014microsoft}
is a large-scale benchmark dataset widely used for various computer vision research problems such as object detection and segmentation. It includes 330k images, among which over 200k of them are labeled. 
In terms of the multimodal attributes, MSCOCO includes the textual captions for each image and therefore can be applied to vision and text related tasks such as image captioning and text-to-image synthesis. 

\noindent \textbf{Conceptual Captions} (CC) dataset~\cite{sharma2018conceptual,changpinyo2021conceptual} provides image-caption pairs extracted from Internet. The training split of the CC dataset has more than 3M images with a token vocabulary size of 51k. Each caption has an average length 10.3 words (tokens). The validation and testing splits include more than 15k images.
As one of the largest open access image-caption datasets, the CC dataset is often used for large-scale model pretraining. 
Note that several large-scale pre-trained models (\textit{e.g.}, CLIP~\cite{radford2021clip}) do not release their training dataset.

\noindent \textbf{CUB200} dataset~\cite{WahCUB_200_2011} contains 11,788 images of 200 bird species. The training and testing splits include 5,994 and 5,794 images respectively. The textual descriptions of each bird image are later annotated by~\cite{reed2016learning}. Compared to the previous large vision and text datasets such as MSCOCO and CC, CUB200 focus on a very specific and fine-grained category of visual information.   

\noindent \textbf{VisDial} dataset~\cite{das2017visual} contains images and the related question answer dialog annotations, which are designed for machines to maintain a meaningful dialog given the visual information as input. The 120k images of VisDial come from MSCOCO and each has a corresponding dialog annotation that consist of 10 question and answer pairs, resulting in 1.2M rounds of dialog interactions. It is a benchmark dataset used for vision and text related tasks such as visual dialog~\cite{das2017visual}.

\noindent \textbf{GuessWhat?!} is a large-scale dataset consisting of 800k visual question and answer pairs on 66k images in total~\cite{de2017guesswhat}.
Specifically, the data are collected from a cooperative two-player game named \textit{GuessWhat?!}, in which both players see the image. 
One player of the game - the oracle - is assigned a random object from the given image, while the other player - the questioner - does not know the target object assigned. The game objective is for the questioner to locate the target object via dialog interactions with the oracle. 
This is a dataset usually applicable in the visual dialog task.

\noindent \textbf{NExT-QA}~\cite{xiao2021next} is a benchmark dataset with videos and question-answer dialog. The main difference of this video-text dataset lies within the fact that the NExT-QA is claimed to host causal and temporal action reasoning in the video question answering process.
It includes a total of 5440 videos with an average length of 44 seconds. For each video, the dataset provides 10 rounds of question and answer pairs as the dialog annotations, resulting in a total of 52k manually labeled question and answer pairs. 
The question and answer pairs are further grouped into clusters with causal, temporal, or descriptive attributes. 

% \yu{there are lots of video-text datasets, such as MSRVTT, MSVD, ActivityNet Captions, VATEX, howto100m.}


\noindent \textbf{MSVD} (Microsoft Research Video Description)~\cite{chen2011collecting} is a dataset consists of about 120K English descriptions for more than 2,000 video clips. It is a dataset first collected and proposed for the machine translation usage, but later also widely used for the video captioning task.


\noindent \textbf{MSR-VTT} (MSR-Video to Text)~\cite{xu2016msr} is a large-sclae video benchmark for video understanding. It contains in total 10,000 web video clips with 41.2 hours and 2000K clip-sentence pairs. Each video clip is annotated with 20 natural sentences. 
MSR-VTT dataset is collected based on 257 popular queries, covering 20 representative categories.
It is mostly adopted in video captioning task.




\noindent \textbf{AVSD} (Audio Visual Scene Aware Dialog)~\cite{hori2019end,alamri2019audio} is a dataset that includes vision, audio and text data attributes. The visual information includes videos from the Charades dataset~\cite{sigurdsson2016hollywood}, and the text data include both caption and dialog annotations. For each dialog of a given video, there are ten rounds of question-answer pairs. This dataset can be applied in both video captioning~\cite{zhu2020describing,zhu2021saying} or video-based question answering~\cite{schwartz2019simple}.

\noindent \textbf{AVE.} (Audio Visual Event) dataset~\cite{tian2018audio} contains 4143 unconstrained 10s videos covering 28 event categories such as dog barking, frying food, and playing guitar.
Most videos contain visual events that span over the full 10 seconds, and the visual event within the video is accompanied by its corresponding ambient sound.
This dataset is proposed to study the audio-visual event localization problems~\cite{tian2018audio,wu2019dual,zhu2021learning}.

\noindent \textbf{AIST}~\cite{aist-dance-db} is a dataset with professional dance videos with paired dance music, which is also one of the first large-scale datasets for street dances. It contains 13,940 videos with 1,618 dances, accompanied by 60 music pieces. The total video length is about 118.1 hours. The dances in the AISTcover 10 different genres such as break, pop, house, and street jazz. 
The dance choreographers are performed by professional dancers and the videos are recorded in a studio environment from 9 camera poses.
This dataset was initially collected for the purpose of promoting dance information processing, but has been later utilized in more cross-modal scenarios related to dance and music.

Additionally, \textbf{AIST++}~\cite{aistplus} is a subset of AIST with more refined dance motion annotations. Specifically, this dataset provides motion annotations in form of Skinkked Multi-Person Linear (SPML) representations~\cite{SMPL:2015}, 3D human body keypoints, and 2D human keypoints, proposed for the music-to-dance generation task~\cite{aistplus} that seek to generate dance motions from given musical audio input.  

\noindent \textbf{TikTok Dance-Music}~\cite{yezhu2022quantizedgan} includes dance videos with paired music collected from the TikTok social platform. This dataset includes 445 video clips with an average length of 12.3 seconds with 85 different songs.
Similar to the AIST++~\cite{aistplus}, it also contains the motion attributes, represented by the 2D human skeleton data.
As another dataset for the dance and music cross-modality generation task, the major difference between AIST++ and TikTok Dance-Music lies within the fact that the former has clearer settings, while the latter is rather ``in the wild", and therefore also more challenging when utilized in concrete dance and music related tasks. 
% since all the dance choreographers are performed by professional dancers and the videos are recorded in studio environment from multiple angles. 

\noindent \textbf{MUSIC}~\cite{zhao2018sound,zhao2019sound} is a dedicated dataset for music instrumental performance videos. It includes 685 untrimmed videos of musical solos and duets with 11 instrumental types such as guitar, cello, and violin. For each video, there is also the corresponding music sound. 
The dataset has been initially proposed for visual-audio grounding problems, such as the spatial sound localization within the videos~\cite{zhao2018sound}.

\noindent \textbf{Flicker 8k} has 8000 natural images with caption descriptions. Each sentence has 5 textual descriptions, resulting in 40000 captions in total. 
The \textbf{Flicker Audio Caption Corpus}~\cite{harwath2015deep} provides the speech audio of the 40000 spoken captions.
As a small dataset with vision, audio and text annotations, it is often used for preliminary experiments for sanity checks in multimodal learning related works.   

\noindent \textbf{Look, Listen, and Parse} (LLP)~\cite{tian2020avvp} is a subset of AudioSet~\cite{gemmeke2017audioset}, which contains 11,849 YouTube video clips categorized into 25 event classes. Each video is 10s length, with a corresponding ambient sound that characterizes at least one specific event such as vehicle sounds or human activities. There are in total 6626 event annotations, among which 4131 for audio and 2495 for the visual, paired with second-wise temporal boundaries. Similar to AVE~\cite{tian2018audio}, this dataset was originally proposed for audio-visual tasks such as audio-visual video parsing (AVVP) (see details in Sec.~\ref{sec:discriminative}).

\vspace{-0.1in}
\subsection{Synthetic Dataset}
\label{subsec:syn_data}

Compared to real-world datasets, synthetic datasets usually include generated data with less noise and are often used for the diagnostic purposes of analyzing the reasoning abilities of model networks. 

\noindent \textbf{CLVER}~\cite{johnson2017clevr} is a diagnostic synthetic dataset for visual reasoning and compositional language parsing. It contains images with geometrical shapes of cubes, cylinders, and spheres in different colors and materials. The main dataset includes 70k, 15k, and 15k images for the training, validation, and test sets, respectively. In addition to the images, CLVER also provides question and answer annotations.

\noindent \textbf{MUGEN}~\cite{hayes2022mugen} is a recently proposed large-scale synthetic dataset for multimodal studies with vision, audio and text data attributes. The data of MUGEN are collected from the open-source platform game CoinRun~\cite{cobbe2019quantifying}, which includes 375k video clips of 3.2 seconds, paired music sequences and corresponding human-annotated text descriptions. 

==> sections/pretraining.tex <==
\section{Large-Scale Pretraining}
\label{sec:pretraining}

Nowadays, there are several large-scale pre-trained models in multimodal learning research area that have been attracting much attention.
On the one hand, such models have achieved 
